Integrating Column Generation and Large Neighborhood Search for Bus Driver Scheduling with Complex Break Constraints

The Bus Driver Scheduling Problem (BDSP) is a combinatorial optimization problem with the goal to design shifts to cover prearranged bus tours. The objective takes into account the operational cost as well as the satisfaction of drivers. This problem is heavily constrained due to strict legal rules and collective agreements. The objective of this article is to provide state-of-the-art exact and hybrid solution methods that can provide high-quality solutions for instances of different sizes. This work presents a comprehensive study of both an exact method, Branch and Price (B&P), as well as a Large Neighborhood Search (LNS) framework which uses B&P or Column Generation (CG) for the repair phase to solve the BDSP. It further proposes and evaluates a novel deeper integration of B&P and LNS, storing the generated columns from the LNS subproblems and reusing them for other subproblems, or to find better global solutions. The article presents a detailed analysis of several components of the solution methods and their impact, including general improvements for the B&P subproblem, which is a high-dimensional Resource Constrained Shortest Path Problem (RCSPP), and the components of the LNS. The evaluation shows that our approach provides new state-of-the-art results for instances of all sizes, including exact solutions for small instances, and low gaps to a known lower bound for mid-sized instances. Conclusions: We observe that B&P provides the best results for small instances, while the tight integration of LNS and CG can provide high-quality solutions for larger instances, further improving over LNS which just uses CG as a black box. The proposed methods are general and can also be applied to other rule sets and related optimization problems

==> bound_bp.tex <==

\begin{table}
\centering
\caption{Lower Bounds with three different versions of Branch And Price.}
\label{tab:bp_lb}
\begin{tabular}{c*{3}{S[table-format=6.2]}}
\toprule
$i$ & {\bpplain}        & {\bpmulti}        & {\bpbg}         \\ 
\midrule
1         & 14417     & 14417     & 14417     \\
2         & 14572     & 14572     & 14572     \\
3         & 15103     & 15103     & 15103     \\
4         & 15148     & 15148     & 15148     \\
5         & 14306     & 14306     & 14306     \\
6         & 30427     & 30427     & 30427     \\
7         & 30576.33  & 30577     & 30578.67  \\
8         & 30437     & 30437     & 30437     \\
9         & 29520     & 29520     & 29520     \\
10        & 30480     & 30480     & 30480     \\
11        & 48667.27  & 48668.84  & 48668.21  \\
12        & 50916.26  & 50924.48  & 50917.46  \\
13        & 50771.35  & 50775.55  & 50775.55  \\
14        & 48441.08  & 48442.75  & 48442     \\
15        & 49547.57  & 49548.86  & 49547.57  \\
16        & 66285.66  & 66298.16  & 66285.66  \\
17        & 67591.41  & 67592.56  & 67591.41  \\
18        & 67051.93  & 67058.99  & 67059.54  \\
19        & 66412.5   & 66420.74  & 66412.7   \\
20        & 66573.94  & 66576.39  & 66573.94  \\
21        & 82614.5   & 82614.5   & 82614.5   \\
22        & 84569.08  & 84575.06  & 84571.62  \\
23        & 83411.18  & 83411.18  & 83411.18  \\
24        & 85319.87  & 85318.85  & 85324.2   \\
25        & 84269.08  & 84273.44  & 84269.08  \\
26        & 99286.72  & 99288.2   & 99286.72  \\
27        & 100328.85 & 100339.69 & 100368.75 \\
28        & 98990.15  & 98990.15  & 98990.15  \\
29        & 98991.82  & 98991.82  & 98991.82 \\
\bottomrule
\end{tabular}
\end{table}
\endinput

==> result_bp.tex <==
\begin{longtable}{l*{3}{S[table-format=5.0, table-model-setup = \bfseries]]S[table-format=1.1]S[table-format=4.1]}}
%
\caption{Comparison of the three variants of BP.\label{tab:results_bp}} \\
%  
\toprule
i &\multicolumn{3}{c}{BP1}&\multicolumn{3}{c}{BP2}&\multicolumn{3}{c}{BP3} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
&  {Best} & {Gap} &{Time} &  {Best} & {Gap} &{Time}&  {Best} & {Gap} &{Time}\\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
1 & \textbf{14417} & 0.00 & 4.8 & \textbf{14417} & 0.00 & 4.4 & \textbf{14417} & 0.00 & 4.8 \\
2 & \textbf{14572} & 0.00 & 11.7 & \textbf{14572} & 0.00 & 10.9 & \textbf{14572} & 0.00 & 11.7 \\
3 & \textbf{15103} & 0.00 & 23.9 & \textbf{15103} & 0.00 & 23.1 & \textbf{15103} & 0.00 & 19.5 \\
4 & \textbf{15148} & 0.00 & 2.4 & \textbf{15148} & 0.00 & 2.1 & \textbf{15148} & 0.00 & 2.2 \\
5 & \textbf{14306} & 0.00 & 1.9 & \textbf{14306} & 0.00 & 1.6 & \textbf{14306} & 0.00 & 1.4 \\
6 & \textbf{30427} & 0.00 & 155.9 & \textbf{30427} & 0.00 & 123.0 & \textbf{30427} & 0.00 & 151.9 \\
7 & 30633 & 0.19 & 3600.0 & 30633 & 0.18 & 3609.4 & \textbf{30609} & 0.10 & 3613.6 \\
8 & \textbf{30437} & 0.00 & 1740.2 & \textbf{30437} & 0.00 & 1547.8 & \textbf{30437} & 0.00 & 1654.1 \\
9 & \textbf{29520} & 0.00 & 44.7 & \textbf{29520} & 0.00 & 41.7 & \textbf{29520} & 0.00 & 42.1 \\
10 & \textbf{30480} & 0.00 & 1609.4 & \textbf{30480} & 0.00 & 1281.5 & \textbf{30480} & 0.00 & 1590.0 \\
11 & \textbf{48754} & 0.18 & 3626.4 & 48762 & 0.19 & 3600.0 & \textbf{48754} & 0.18 & 3601.1 \\
12 & \textbf{51115} & 0.39 & 3600.0 & \textbf{51115} & 0.37 & 3600.0 & \textbf{51115} & 0.39 & 3601.1 \\
13 & \textbf{50962} & 0.38 & 3600.1 & \textbf{50962} & 0.37 & 3620.2 & \textbf{50962} & 0.37 & 3620.5 \\
14 & \textbf{48779} & 0.70 & 3600.0 & \textbf{48779} & 0.69 & 3602.0 & \textbf{48779} & 0.70 & 3601.0 \\
15 & \textbf{49622} & 0.15 & 3600.0 & \textbf{49622} & 0.15 & 3600.0 & \textbf{49622} & 0.15 & 3605.1 \\
16 & \textbf{66420} & 0.20 & 3600.2 & 66443 & 0.22 & 3600.4 & \textbf{66420} & 0.20 & 3601.6 \\
17 & 67695 & 0.15 & 3642.8 & \textbf{67692} & 0.15 & 3600.1 & \textbf{67692} & 0.15 & 3601.1 \\
18 & \textbf{67448} & 0.59 & 3600.7 & 67450 & 0.58 & 3600.0 & \textbf{67448} & 0.58 & 3601.1 \\
19 & \textbf{66478} & 0.10 & 3600.3 & \textbf{66478} & 0.09 & 3600.1 & \textbf{66478} & 0.10 & 3601.0 \\
20 & 67044 & 0.71 & 3618.3 & \textbf{66983} & 0.61 & 3600.3 & 67044 & 0.71 & 3615.7 \\
21 & \textbf{83148} & 0.65 & 3603.9 & \textbf{83148} & 0.65 & 3600.1 & \textbf{83148} & 0.65 & 3602.4 \\
22 & \textbf{84836} & 0.32 & 3600.1 & \textbf{84836} & 0.31 & 3600.3 & \textbf{84836} & 0.31 & 3717.5 \\
23 & \textbf{83599} & 0.23 & 3600.3 & 83638 & 0.27 & 3601.2 & \textbf{83599} & 0.23 & 3612.0 \\
24 & \textbf{85610} & 0.34 & 3734.1 & \textbf{85610} & 0.34 & 3613.9 & \textbf{85610} & 0.33 & 3601.1 \\
25 & 84501 & 0.28 & 3600.2 & 84492 & 0.26 & 3600.1 & \textbf{84469} & 0.24 & 3601.1 \\
26 & \textbf{99403} & 0.12 & 3600.3 & \textbf{99403} & 0.12 & 3693.9 & \textbf{99403} & 0.12 & 3601.1 \\
27 & 101322 & 0.99 & 5636.6 & 101322 & 0.98 & 3600.4 & \textbf{101151} & 0.78 & 3601.1 \\
28 & \textbf{99170} & 0.18 & 3600.0 & \textbf{99170} & 0.18 & 3600.4 & \textbf{99170} & 0.18 & 3602.3 \\
29 & \textbf{99433} & 0.45 & 3601.0 & \textbf{99433} & 0.45 & 3600.6 & \textbf{99433} & 0.45 & 3601.1 \\
30 & \textbf{99445} & {inf} & 3854.8 & \textbf{99445} & {inf} & 3672.9 & \textbf{99445} & {inf} & 3605.9 \\
31 & 117130 & {inf} & 4506.6 & \textbf{116991} & {inf} & 3742.4 & 117463 & {inf} & 3601.2 \\
32 & \textbf{118463} & {inf} & 3688.8 & \textbf{118463} & {inf} & 3635.8 & 118472 & {inf} & 3601.2 \\
33 & 119026 & {inf} & 7200.9 & \textbf{118970} & {inf} & 7200.6 & 119109 & {inf} & 3602.2 \\
34 & 118832 & {inf} & 7200.2 & \textbf{118796} & {inf} & 5756.8 & 119055 & {inf} & 3601.3 \\
35 & 118237 & {inf} & 7200.2 & \textbf{118208} & {inf} & 5403.2 & 118265 & {inf} & 3601.5 \\
36 & 134308 & {inf} & 5832.7 & \textbf{134115} & {inf} & 3858.9 & 134308 & {inf} & 3601.2 \\
37 & 134544 & {inf} & 7201.1 & \textbf{134482} & {inf} & 7200.6 & 134585 & {inf} & 3601.1 \\
38 & \textbf{135348} & {inf} & 3786.4 & \textbf{135348} & {inf} & 3694.6 & 135534 & {inf} & 3601.1 \\
39 & 136730 & {inf} & 7200.2 & \textbf{135740} & {inf} & 5983.3 & 136748 & {inf} & 3601.3 \\
40 & 133699 & {inf} & 7201.4 & \textbf{133620} & {inf} & 5478.2 & 133715 & {inf} & 3602.7 \\
41 & 149515 & {inf} & 7200.4 & \textbf{149508} & {inf} & 7200.4 & 149658 & {inf} & 3601.1 \\
42 & 150655 & {inf} & 7200.3 & \textbf{150329} & {inf} & 7200.3 & 150770 & {inf} & 3602.8 \\
43 & 150890 & {inf} & 7200.7 & \textbf{150745} & {inf} & 7200.9 & 151049 & {inf} & 3601.3 \\
44 & \textbf{149508} & {inf} & 7200.6 & \textbf{149508} & {inf} & 5362.9 & 151182 & {inf} & 3601.6 \\
45 & 150896 & {inf} & 7202.6 & \textbf{150770} & {inf} & 7200.8 & 151364 & {inf} & 3601.5 \\
46 & 175040 & {inf} & 7201.2 & \textbf{172574} & {inf} & 7200.3 & 175845 & {inf} & 3601.5 \\
47 & 165210 & {inf} & 4320.1 & \textbf{165201} & {inf} & 3965.8 & 165210 & {inf} & 3601.6 \\
48 & \textbf{168153} & {inf} & 7200.2 & 168204 & {inf} & 7200.4 & 174747 & {inf} & 3601.4 \\
49 & 169039 & {inf} & 7200.8 & \textbf{168865} & {inf} & 7202.4 & 169021 & {inf} & 3601.5 \\
50 & 165329 & {inf} & 7200.6 & \textbf{165278} & {inf} & 5938.2 & 165527 & {inf} & 3601.2 \\
51 & 266077 & {inf} & 7200.3 & \textbf{261279} & {inf} & 7200.4 & 270624 & {inf} & 3601.4 \\
52 & 272349 & {inf} & 7200.8 & \textbf{271552} & {inf} & 7200.9 & 281092 & {inf} & 3601.4 \\
53 & 274263 & {inf} & 7200.3 & \textbf{267272} & {inf} & 7200.5 & 281737 & {inf} & 3602.0 \\
54 & 273700 & {inf} & 7200.3 & \textbf{264955} & {inf} & 7200.3 & 286486 & {inf} & 3601.9 \\
55 & 281757 & {inf} & 7200.4 & \textbf{267268} & {inf} & 7200.4 & 284743 & {inf} & 3601.2 \\
56 & 380098 & {inf} & 7200.7 & \textbf{357927} & {inf} & 7200.8 & 390807 & {inf} & 3601.3 \\
57 & 389369 & {inf} & 7200.3 & \textbf{374936} & {inf} & 7200.6 & 394994 & {inf} & 3610.9 \\
58 & \textbf{375230} & {inf} & 7200.5 & 382323 & {inf} & 7200.5 & 382374 & {inf} & 3603.5 \\
59 & \textbf{373198} & {inf} & 7205.0 & 373584 & {inf} & 7200.6 & 390973 & {inf} & 3601.3 \\
60 & 384695 & {inf} & 7203.8 & \textbf{370940} & {inf} & 7200.4 & 395559 & {inf} & 3601.7 \\
61 & 554480 & {inf} & 7228.6 & \textbf{495987} & {inf} & 7205.1 & 554342 & {inf} & 3601.3 \\
62 & \textbf{501445} & {inf} & 7200.4 & 507461 & {inf} & 7217.8 & 557993 & {inf} & 3603.2 \\
63 & \textbf{495152} & {inf} & 7257.5 & 496015 & {inf} & 7212.0 & 499972 & {inf} & 3601.6 \\
64 & 515030 & {inf} & 7202.0 & \textbf{482069} & {inf} & 7206.8 & 497706 & {inf} & 3607.9 \\
65 & 534210 & {inf} & 7200.5 & \textbf{509080} & {inf} & 7200.5 & 564673 & {inf} & 3601.5 \\
\end{longtable}
\endinput % Facoltativo ma utile

==> result_table.tex <==
\begin{longtable}[htp]{l*{3}{S[table-format=6.0]S[table-format=6.1, table-model-setup = \bfseries]}S[table-format=6, table-model-setup = \bfseries]}
\caption{Aggregated main results.} \label{tab:results} \\
\toprule
$i$ & plain min & plain avg & cs\_bg\_full min & cs\_bg\_full avg & CMSA min & CMSA avg & BP \\
\midrule
\endfirsthead
\caption[]{Aggregated main results.} \\
\toprule
$i$ & plain min & plain avg & cs\_bg\_full min & cs\_bg\_full avg & CMSA min & CMSA avg & BP \\
\midrule
\endhead
\midrule
\multicolumn{8}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
1 & 14417 & \bfseries 14417.0 & 14417 & \bfseries 14417.0 & 14530 & 14549.0 & \bfseries 14417 \\
2 & 14572 & \bfseries 14572.0 & 14572 & 14573.0 & 14655 & 14655.0 & \bfseries 14572 \\
3 & 15103 & \bfseries 15103.0 & 15103 & 15196.9 & 15381 & 15381.0 & \bfseries 15103 \\
4 & 15148 & \bfseries 15148.0 & 15148 & \bfseries 15148.0 & 15148 & 15187.9 & \bfseries 15148 \\
5 & 14306 & \bfseries 14306.0 & 14306 & \bfseries 14306.0 & 14623 & 14625.7 & \bfseries 14306 \\
6 & 30427 & 30450.2 & 30427 & \bfseries 30427.0 & 30820 & 30862.0 & \bfseries 30427 \\
7 & 30609 & 30619.2 & 30609 & 30615.5 & 31038 & 31091.5 & \bfseries 30610 \\
8 & 30437 & 30491.3 & 30437 & \bfseries 30437.0 & 30962 & 31022.4 & \bfseries 30437 \\
9 & 29520 & \bfseries 29520.0 & 29520 & \bfseries 29520.0 & 29882 & 29943.9 & \bfseries 29520 \\
10 & 30480 & 30480.7 & 30480 & \bfseries 30480.0 & 30777 & 30809.8 & \bfseries 30480 \\
11 & 48764 & 48904.9 & 48731 & 48736.2 & 49577 & 49665.2 & \bfseries 48731 \\
12 & 51211 & 51282.7 & 51115 & 51135.9 & 52074 & 52194.9 & \bfseries 51115 \\
13 & 50962 & 51057.9 & 50962 & \bfseries 50962.0 & 51864 & 51931.3 & \bfseries 50962 \\
14 & 48776 & 48854.5 & 48775 & \bfseries 48799.9 & 49429 & 49545.4 & 48802 \\
15 & 49622 & 49732.2 & 49622 & \bfseries 49622.0 & 50713 & 50749.2 & \bfseries 49622 \\
16 & 66451 & 66598.8 & 66400 & \bfseries 66404.5 & 67840 & 67962.0 & 66417 \\
17 & 67858 & 67982.8 & 67692 & 67698.1 & 69338 & 69475.3 & \bfseries 67695 \\
18 & 67389 & 67490.5 & 67300 & \bfseries 67323.0 & 68827 & 68915.7 & 67424 \\
19 & 66498 & 66613.1 & 66478 & 66486.3 & 67582 & 67659.5 & \bfseries 66478 \\
20 & 66923 & 67143.4 & 66918 & \bfseries 66921.5 & 68387 & 68487.2 & 66988 \\
21 & 83089 & 83188.9 & 82936 & \bfseries 82940.1 & 85119 & 85332.3 & 83148 \\
22 & 84921 & 85221.1 & 84778 & \bfseries 84805.9 & 86623 & 86768.7 & 84836 \\
23 & 83721 & 83814.5 & 83594 & 83605.3 & 85389 & 85473.9 & \bfseries 83595 \\
24 & 85799 & 85946.0 & 85579 & \bfseries 85596.1 & 87412 & 87661.1 & 85628 \\
25 & 84547 & 84747.9 & 84370 & \bfseries 84413.4 & 86552 & 86710.0 & 84498 \\
26 & 99617 & 99746.9 & 99403 & 99415.5 & 101204 & 101368.4 & \bfseries 99403 \\
27 & 101274 & 101534.6 & 101024 & \bfseries 101082.8 & 104982 & 105492.5 & 101209 \\
28 & 99718 & 100159.8 & 99272 & 99320.5 & 102538 & 102642.7 & \bfseries 99178 \\
29 & 99635 & 99823.5 & 99339 & \bfseries 99349.9 & 102173 & 102324.0 & 99373 \\
30 & 99788 & 99967.0 & 99330 & \bfseries 99355.0 & 102084 & 102286.7 & 99472 \\
31 & 117142 & 117242.1 & 116592 & \bfseries 116635.6 & 119308 & 119530.5 & 116863 \\
32 & 118930 & 119045.3 & 118441 & 118478.6 & 121460 & 121636.4 & \bfseries 118472 \\
33 & 118933 & 119158.3 & 118318 & \bfseries 118475.8 & 121138 & 121370.1 & 119454 \\
34 & 119098 & 119335.4 & 118580 & \bfseries 118614.3 & 121736 & 121905.0 & 118983 \\
35 & 118458 & 118713.2 & 118025 & \bfseries 118052.2 & 121036 & 121267.5 & 118849 \\
36 & 133854 & 134171.2 & 133127 & \bfseries 133200.9 & 136817 & 137005.2 & 133384 \\
37 & 134493 & 135034.6 & 133661 & \bfseries 133774.3 & 137944 & 138603.6 & 134813 \\
38 & 135932 & 136291.3 & 135299 & 135369.2 & 139094 & 139278.7 & \bfseries 135354 \\
39 & 136057 & 136384.9 & 135143 & \bfseries 135254.0 & 141245 & 141716.3 & 135508 \\
40 & 133802 & 134012.1 & 132687 & \bfseries 132809.4 & 136934 & 137197.5 & 133510 \\
41 & 149190 & 149697.9 & 148488 & \bfseries 148677.7 & 152977 & 153291.7 & 149342 \\
42 & 150642 & 150936.9 & 149859 & \bfseries 149928.8 & 154906 & 155572.6 & 149985 \\
43 & 150521 & 151135.7 & 150053 & \bfseries 150245.7 & 155595 & 156074.1 & 151246 \\
44 & 149843 & 150227.8 & 148185 & \bfseries 148341.7 & 154984 & 155243.6 & 149956 \\
45 & 151217 & 151609.5 & 150116 & \bfseries 150278.3 & 155001 & 155209.4 & 151325 \\
46 & 165697 & 165934.5 & 164451 & \bfseries 165218.2 & 170593 & 171648.9 & 184186 \\
47 & 165176 & 165878.6 & 164381 & \bfseries 164410.1 & 169992 & 170308.2 & 165268 \\
48 & 167265 & 167601.2 & 166310 & \bfseries 166629.7 & 171738 & 172175.8 & 176430 \\
49 & 168557 & 169087.6 & 167394 & \bfseries 167869.7 & 173986 & 174890.4 & 171275 \\
50 & 165292 & 165555.8 & 164121 & \bfseries 164366.7 & 169488 & 169910.3 & 165752 \\
51 & 251250 & 251893.3 & 250478 & \bfseries 251371.1 & 258908 & 259303.4 & NaN \\
52 & 257048 & 257736.5 & 256206 & \bfseries 256933.5 & 265643 & 266014.9 & NaN \\
53 & 255521 & 256570.1 & 255763 & \bfseries 256391.9 & 265714 & 265973.2 & NaN \\
54 & 256103 & 256506.5 & 255008 & \bfseries 256159.7 & 263511 & 263784.5 & NaN \\
55 & 253789 & 254539.2 & 253524 & \bfseries 254231.7 & 261620 & 261862.7 & NaN \\
56 & 339133 & \bfseries 339912.9 & 338966 & 340267.9 & 351189 & 351551.0 & NaN \\
57 & 339400 & 340397.6 & 339736 & \bfseries 340261.8 & 350191 & 350679.6 & NaN \\
58 & 336049 & 336410.5 & 335751 & \bfseries 336313.3 & 346885 & 347150.4 & NaN \\
59 & 336657 & \bfseries 337615.7 & 336242 & 337690.7 & 348357 & 348841.5 & NaN \\
60 & 336156 & 336797.7 & 335414 & \bfseries 336272.1 & 346421 & 346862.7 & NaN \\
61 & 426676 & 427603.7 & 425880 & \bfseries 426806.8 & 437522 & 438010.0 & NaN \\
62 & 427686 & \bfseries 428522.7 & 428008 & 428680.4 & 440515 & 440913.8 & NaN \\
63 & 426333 & \bfseries 427514.6 & 426919 & 427740.5 & 438561 & 438968.3 & NaN \\
64 & 428442 & \bfseries 429295.8 & 427983 & 429352.1 & 440638 & 440934.7 & NaN \\
65 & 425405 & \bfseries 426396.6 & 424907 & 426440.1 & 436821 & 437345.5 & NaN \\
\end{longtable}

